UVSCAN: Detecting Third-Party Component Usage Violations in IoT Firmware

Nowadays, IoT devices integrate a wealth of third-party components (TPCs) in firmware to shorten the development cycle. TPCs usually have strict usage specifications, e.g., checking the return value of the function. Violating the usage specifications of TPCs can cause serious consequences, e.g., NULL pointer dereference. Therefore, this massive amount of TPC integrations, if not properly implemented, will lead to pervasive vulnerabilities in IoT devices. Detecting vulnerabilities automatically in TPC integration is challenging from several perspectives: (1) There is a gap between the high-level specifications from TPC documents, and the low-level implementations in the IoT firmware. (2) IoT firmware is mostly the closed-source binary, which loses a lot of information when compiling from the source code and has diverse architectures. To address these challenges, we design and implement UVScan, an automated and scalable system to detect TPC usage violations in IoT firmware. In UVScan, we first propose a novel natural language processing (NLP)-based rule extraction framework, which extracts API specifications from inconsistently formatted TPC documents. We then design a rule-driven NLP-guided binary analysis engine, which maps the logical information from the high-level TPC document to the low-level binary, and detects TPC usage violations in IoT firmware across different architectures. We evaluate UVScan from four perspectives on four popular TPCs and six ground-truth datasets. The results show that UVScan achieves more than 70% precision and recall, and has a significant performance improvement compared with even the source-level API misuse detectors.

==> 0x0Challenges.tex <==
% \section{Overview}


==> 0x0Evaluation.tex <==
\vspace{-1em}
% \section{\textcolor{red}{System Evaluation}}
\section{System Evaluation}
\label{section: System Evaluation}
% In this section, we mainly evaluate the performance of \system. 
% Though the goal of this paper is not to propose a novel method, we want to convince people that the measurement results based on \system are reliable through the evaluation. % 
In this section, we first introduce the composition of the dataset ~\Footnotes\footnote{We provide some information about the firmware in our dataset on https://github.com/FirmSecDataset/FirmSecDataset.}, which will be used in system evaluation and further large-scale analysis. Next, we evaluate the performance of \system, and compare it with state-of-the-art  works  from  academia  and  commercial  systems  from  industry: \textit{Gemini}~\cite{xu2017neural}, \textit{BAT}~\cite{hemel2011finding},  \textit{OSSPolice}~\cite{duan2017identifying}, \textit{binaré}~\cite{binare}, \textit{360 FirmwareTotal}~\cite{360iot}, and \textit{Alibaba FSS}~\cite{aliiot}.
% evaluate the accuracy of \system which achieves 
% % $100\%$ accuracy in identifying TPCs and 
% $96.3\%$  in discovering corresponding vulnerabilities. 
% % Then, we perform the \system on our dataset which identifies $584$ TPCs and discovers a total of $128,757$ security vulnerabilities that are caused by $429$ CVEs. 
% Then,  we compare \system with one academic system developed by Costin et al.~\cite{costin2014large}, and two industry-leading systems from \textit{360}~\cite{360iot} and \textit{Alibaba}~\cite{aliiot}. 
% \system detects an average of $15.8$ TPCs and $114.2$ vulnerabilities per firmware image while the corresponding results of \cite{costin2014large}, \textit{360}, and \textit{Alibaba} are $7.7$ and $82.9$, $4.8$ and $62.3$, and $3$ and $55.5$, respectively. In addition, \system spends an average of $4.2s$ processing each firmware while \cite{costin2014large} spends $303s$, \textit{360} spends $60s$, and \textit{Alibaba} spends $174.7s$.
% \system is eligible to identify more TPCs and discover more corresponding vulnerabilities based on the same vulnerability database that faster than 360~\cite{360iot} and \textit{Alibaba}~\cite{aliiot}. 




\vspace{-2mm}
\subsection{Dataset Composition}
\label{subsection: Dataset Composition}
Based on the firmware collection module, we initially collect a total of %$37,266$%  
$35,978$ firmware images varying from $13$ vendors which involve $35$ kinds of devices. More specifically, %$13,328$% 
$12,913$ firmware images are crawled from the Internet and %$23,938$%
$23,065$ firmware images are obtained from TSmart. Our dataset actually involves hundreds of vendors since the private firmware images from TSmart are manufactured by hundreds of vendors. TSmart provides a platform that can enable the devices from various vendors to become smart products. We use TSmart as the vendor of private firmware for convenience. 
% Next, we filter the non-firmware files from our raw dataset and identify the related information of remaining unrecognized firmware, according to the firmware preprocessing module. 
We list the detailed composition of our dataset as shown in Table~\ref{Table: Dataset Composition} (Appendix~\ref{section: Vulnerability Evaluation}). 
After data filtration, we get rid of %$2,770$%
$1,842$ non-firmware files and finally obtain %$33,833$%
$34,136$ valid firmware images across $13$ vendors including %$13,173$%
$11,086$ publicly accessible firmware images and 
%$23,430$% 
$23,050$ private firmware images from TSmart. 
Our dataset includes  $35$ kinds of known IoT devices and a part of unknown IoT devices.  $2,694$ ($7.9\%$) firmware images are used in camera, $7,293$ ($21.3\%$) firmware images belong to router, $1,191$ ($3.5\%$) firmware images are deployed on switch, $23,050$ ($67.5\%$) firmware images from TSmart have been equipped on smart homes, and $255$ ($0.7\%$) are unknown firmware images.
% , and $401$ ($1.2\%$) firmware images are from other kinds of devices.
% However, there are still $1,249$ ($3.7\%$) firmware images whose exact device categories cannot be identified. We classify these unidentified firmware images as unknown. 
Apart from the vendors and devices mentioned above, our dataset also covers several instruction sets, of which ARM ($23.9\%$) takes the majority and MIPS follows ($4.9\%$). SquashFS, CramFS, and JFFS2 are three popular filesystems included in the dataset.  Most of the unknown filesystems actually belong to the above three filesystems based on our further analysis. Vendors customize the above filesystems in firmware, which also changes the magic number of original filesystems used for identification. Moreover, 12,342 ($36.2\%$) firmware images are Linux-based and 21,794 ($63.8\%$) firmware images are non-Linux based. All non-Linux based firmware images are from TSmart.

% Some different filesystems are also included in the dataset, like SquashFS, CramFS and etc. 
% Besides, little endian is mostly adopted in the firmware.
% Despite that the embedded system environment is heterogeneous, spanning a variety of devices, vendors, architectures, instruction sets, operating systems, and custom components, we spare no efforts to build a more representative dataset.






Overall, our firmware dataset is highly representative which contains IoT devices ranging from consumer to professional devices, such as router, camera, switch, smart homes, open-source firmware and so on. Besides, the dataset includes a great number of private firmware images, which are used for research purposes for the first time. Our dataset has a larger scale and higher research value than previous studies. To facilitate  future  firmware  security research, we will open-source our dataset.


% \begin{table}[]
% \centering
% \caption{Accuracy Evaluation of \system.}
% % \setlength{\belowcaptionskip}{10pt}
% \vspace{-1mm}
% \tiny
% \renewcommand\arraystretch{0.9}
% \resizebox{0.5\textwidth}{!}{
% \label{Table: Accuracy Evaluation}
% \begin{tabular}{ccccc}
% \hline \hline
% Vendor   & Category     & Firmware                          & \# Vul. & \# Verified  Vul. \\ \hline
% Trendnet & Router       & openwrt-ar71xx-generic-823dru.bin & 21      & 21                \\
% Trendnet & Router       & tew-654tr\_a1\_fw100b19.bin       & 19      & 19                \\
% Trendnet & Router       & TEW-638APBV2\_V1.1.10.BIN         & 5       & 5                 \\
% Trendnet & Camera       & FW\_344345\_V1.2.2\_20170207.BIN  & 1       & 1                 \\
% Trendnet & Switch       & TEG-082WS-1.00.12-ALL.HEX         & 23      & 23                \\
% TP-Link  & Router       & wr810nv2\_eu\_boot(160509).bin    & 24      & 24                \\
% TP-Link  & Router       & TL-R4149GV1.BIN                   & 56      & 51                \\
% TP-Link  & Router       & ARCHER\_D20V1\_0.8.0.BIN          & 7       & 7                 \\
% TP-Link  & Router       & TL-WR802NV4\_EU\_0.9.1\_3.16.BIN  & 5       & 5                 \\
% TP-Link  & Router       & MR10UV1.BIN                       & 2       & 2                 \\
% TP-Link  & Camera       & NC230\_1.2.1.BIN                  & 9       & 9                 \\
% D-Link   & Router       & DIR-605L\_206B01.BIN              & 4       & 4                 \\
% D-Link   & Router       & DIR100A1\_FW114CNB01.BIX          & 4       & 4                 \\
% D-Link   & Camera       & DCS-932L\_REVB\_V2.12.01.BIN      & 5       & 5                 \\
% D-Link   & Camera       & DCS-800L\_A1\_V1.06.10.BIN        & 16      & 16                \\
% Xiongmai & Camera       & GENERAL\_HZXM\_IPC.BIN            & 2       & 2                 \\
% Xiongmai & Camera       & xmjp\_liteos\_v1.01.bin           & 24      & 24                \\
% Dahua    & Camera       & UPALL\_IPC.BIN                    & 2       & 2                 \\
% Phicomm  & Camera       & PHICOMM\_ROUTER.BIN               & 8       & 8                 \\
% OpenWrt  & Router       & OpenWrt-Router-1.bin              & 9       & 9                 \\
% OpenWrt  & Router       & OpenWrt-Router-2.bin              & 11       & 11                 \\
% OpenWrt  & Router       & OpenWrt-Router-3.bin              & 10       & 10                 \\
% OpenWrt  & Router       & OpenWrt-Router-4.bin              & 10       & 10                 \\
% OpenWrt  & Router       & OpenWrt-Router-5.bin              & 7       & 7                 \\
% TSmart   & Camera       & ipcam.20190314.v02.bin            & 20      & 14                \\
% TSmart   & Camera       & PPSTRONG-2.1.2.BIN                & 6       & 6                 \\
% TSmart   & Camera       & ppstrong-c2-atlantic.bin          & 6       & 6                 \\
% TSmart   & Camera       & PPSTRONG-C2-TSMART.bin            & 7       & 7                 \\
% TSmart   & Camera       & CHMI-CAMERA.BIN                   & 2       & 2                 \\
% TSmart   & Camera       & DIFF-OTA-4.0.7.2017112719.BIN     & 2       & 2                 \\
% TSmart   & Gateway      & TSMART\_RTL8196E\_GW.BIN          & 5       & 5                 \\
% TSmart   & Doorbell     & HANKE-DOORBELL.BIN                & 5       & 5                 \\
% TSmart   & Story Bot    & XR871\_STORYBOT\_QIO.BIN          & 14      & 13                \\
% TSmart   & Light        & YMSMART-2.0.2.BIN                 & 21      & 19                \\
% TSmart   & Sweeper & YY5EV2TP6C\_0.BIN                 & 10      & 10 \\ \hline \hline
% \end{tabular}
% }
% % \vspace{-7em}
% \end{table}


\vspace{-2mm}
\subsection{Evaluation}
\label{section: Accuracy Evaluation}
% \subsubsection{End-to-End Accuracy}
% Before we perform \system on our dataset, it is important to obtain the ground truth that whether the results generated by \system are correct at first. 

% in identifying the TPCs and .
% vulnerabilities caused by TPCs in firmware.


% Though there are some systems~\cite{backes2016reliable,duan2017identifying,zhang2019libid} that have been proposed to detect the TPCs used in Android apps, they cannot analyze the IoT firmware. These systems require Android features support. Besides, there is no 
% We finally compare \system with BAT, Both \textit{Gemini}


\noindent\textbf{Ground-truth Dataset Construction.}    We first build
two ground-truth datasets: (1) Dataset \uppercase\expandafter{\romannumeral1} for choosing the appropriate thresholds used in  \system ; (2) Dataset \uppercase\expandafter{\romannumeral2} for evaluating the accuracy of \system in detecting the TPCs at TPC-level and version-level in firmware. 
These datasets have a labeled mapping of firmware to TPCs usage for ground truth. To the best of our knowledge, there are no such datasets available from previous works. Given it is difficult to know the specific TPCs used in commercial firmware, we finally use OpenWrt firmware images to build our datasets since they have source code and clearly indicate the adopted TPCs with exact versions in the  configuration files. For \textit{Dataset \uppercase\expandafter{\romannumeral1}}, we randomly collect $300$ OpenWrt firmware images from our dataset, which include $17,918$ TPC-version pairs ($73$ different TPCs with $211$ different versions).  For \textit{Dataset \uppercase\expandafter{\romannumeral2}}, we also randomly select $300$ OpenWrt firmware images from our dataset, which include $19,645$ TPC-version pairs ($92$ different TPCs with $194$ different versions).
 We use two datasets to perform the threshold selection and evaluation respectively to avoid bias.


% \noindent$\bullet$\textit{Dataset \uppercase\expandafter{\romannumeral1}}: We first need to construct a dataset e. 

% \noindent$\bullet$\textit{Dataset \uppercase\expandafter{\romannumeral2}}: This dataset includes the firmware which has the confirmed vulnerabilities. We mainly evaluate \system on two vulnerabilities: OpenSSL Heartbleed vulnerability (CVE-2014-0160) and glibc Ghost  vulnerability (CVE-2015-0235). For each vulnerability, we collect $30$ vulnerable firmware images based on manual analysis.

% We first build a ground-truth dataset to evaluate the accuracy of \system in detecting the TPCs used in firmware. This dataset has a labeled mapping of firmware to TPCs usage for ground truth. To the best of our knowledge, there is no such a dataset available from previous works. Given it is difficult to know the specific TPCs used in commercial firmware, we finally collect $300$ OpenWrt firmware images. These open-source firmware images have source code and clearly indicate the adopted TPCs with exact versions in the  configuration files. More specifically, these $300$ firmware images include $72$ different TPCs with $194$ different versions. 

\noindent\textbf{Threshold Selection.}   Our final results are the union of the results that matched by syntactical features and CFG features. We do not directly use the thresholds when the respective method achieves the optimal performance since the union results may not reach the best at this time. We take three thresholds as a whole and utilize the true positive rate (TPR) at version-level as the metric to select the appropriate thresholds. We combine the three thresholds and their corresponding TPR as a four-dimensional vector: [$\alpha$, $\beta$, $\gamma$, TPR]. Each threshold ranges from 0.01 to 1.00. We select the thresholds when the TPR reaches the highest. Based on our experiment, \system achieves the highest TPR (91.47\%) when the thresholds of $D(S_{TPC},S_{Firmware})$, $\frac{S_{TPC}\cap S_{Firmware}}{S_{TPC}}$, and $Sim(ACFG_{TPC}, ACFG_{Firmware})$  are 0.74, 0.52, and 0.64, respectively. We leverage the above thresholds for the following evaluation and analysis.

% two datasets: (1) Dataset \uppercase\expandafter{\romannumeral1} for evaluating the accuracy of \system in detecting the TPCs at version level in firmware; (2) Dataset \uppercase\expandafter{\romannumeral2} for evaluating the accuracy of \system in detecting the specific vulnerabilities in firmware.

% \noindent$\bullet$\textit{Dataset \uppercase\expandafter{\romannumeral1}}: We first need to construct a dataset e. 

% \noindent$\bullet$\textit{Dataset \uppercase\expandafter{\romannumeral2}}: This dataset includes the firmware which has the confirmed vulnerabilities. We mainly evaluate \system on two vulnerabilities: OpenSSL Heartbleed vulnerability (CVE-2014-0160) and glibc Ghost  vulnerability (CVE-2015-0235). For each vulnerability, we collect $30$ vulnerable firmware images based on manual analysis.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{Comparison of \system, \textit{Gemini}, \textit{BAT}, and \textit{OSSPolice}.}
\renewcommand\arraystretch{0.9}
\small
\label{Table: Academic Comparison}
\centering
\begin{tabular}{ccccc}
% 
\hline \hline
\multirow{2}{*}{Tools} & \multicolumn{2}{c}{TPC-level} & \multicolumn{2}{c}{Version-level} \\ \cline{2-5} 
                       & Precision      & Recall       & Precision        & Recall         \\ \hline
\system              & 92.09\%        & 95.24\%      & 91.03\%          & 92.26\%        \\
Syntax-based              & 92.38\%        & 86.29\%      & 91.47\%          & 81.66\%        \\
CFG-based              & 93.72\%        & 82.76\%      & 94.65\%          & 80.90\%        \\
\textit{Gemini}~\cite{xu2017neural}              & 89.60\%        & 74.19\%      & 90.78\%          & 71.73\%        \\
\textit{BAT}~\cite{hemel2011finding}                    & 70.74\%        & 56.38\%      & NA               & NA             \\
\textit{OSSPolice}~\cite{duan2017identifying}              & 86.63\%        & 71.85\%      & 82.51\%          & 67.05\%        \\ \hline \hline
% \textit{Asm2Vec}
\end{tabular}
\vspace{-2em}
\end{table}


\noindent\textbf{Evaluation Results.}   We evaluate the detection accuracy of \system on Dataset \uppercase\expandafter{\romannumeral2} at TPC-level and version-level with two evaluation metrics: precision ($\frac{TP}{TP+FP}$) and recall ($\frac{TP}{TP+FN}$). The false positives represent the TPCs and versions that we wrongly identified, and the false negatives represent the TPCs and versions that we do not find. As shown in Table~\ref{Table: Academic Comparison}, \system achieves $92.09\%$ precision, $95.24\%$ recall at TPC-level, and $91.03\%$ precision, $92.26\%$ recall at version-level. We also list the syntax-based matching results and the CFG-based matching results when the TPR of each method reaches the highest. We find that the precision of the union results is very close to the respective methods, but the recall rate is much higher. We explore the reasons that why the union results have a great performance than the separate methods. First, the true positives of the two methods have non-overlapping parts, thus reducing the union results' false negatives. For instance, the syntax-based method is hard to detect the TPCs which have limited syntactical features (e.g., without unique string literals), but they can be identified through CFG features. Second, their false positives have overlapping parts, which will not greatly increase the false positives of the union results. We further analyze the false positives and false negatives. First, the false positives are mainly caused by two reasons: 1) TPCs overlapping. We find several TPCs reuse the code of other TPCs with minor changes. Under these circumstances, \system will report all matched TPCs. 2) High similarity between different versions. Some versions of the same TPC have little difference or even no difference in their code. Second, the false negatives are due to two reasons: 1) Uncommon TPCs used in firmware. \system cannot detect the TPCs that are not included in our database. 2) Insufficient features. Some firmware images only use partially built TPCs which have limited features that can be used for identification.

We also evaluate the  precision of  \system in identifying the vulnerabilities caused by TPCs in firmware, which is discussed in Appendix~\ref{section: Vulnerability Evaluation}.

% For TPC-level, we find the false positives are mainly caused by the reuse of TPCs. Some TPCs reuse the TPCs The false negatives are mainly caused by the high similarity between 
% At TPCs level, we find
% First, we find the little difference between the different versions of TPCs is the main cause for false positives.
% , and the partially built TPCs are the main causes for false positives and false negatives, respectively.


% (1)  
% (2) We perform our test on Dataset \uppercase\expandafter{\romannumeral2} with the retrained model. We retrain the model on  CVE-2014-0160 and CVE-2015-0235 for 10 iterations and each iteration has 5 epochs. For CVE-2014-0160, \system successfully discovers the vulnerability from 29 (96.7\%) firmware images; for CVE-2015-0235, \system finds 27 (90.0\%) firmware images have the vulnerability. These results show that \system has high accuracy in detecting specific vulnerabilities.

% \noindent$\bullet$\textit{Dataset \uppercase\expandafter{\romannumeral1}}: We 

% employ three methods to verify the vulnerabilities: 1) use source code audit to check the vulnerabilities if the source code of the firmware is available; 2) utilize static analysis to verify the vulnerabilities which have disclosed the vulnerable code snippets; and 3) adopt emulating-based dynamic analysis to verify the vulnerabilities which have public Proof-of-Checks (PoCs). We 
% choose these methods for three reasons. First of all, a part of firmware  from OpenWrt has source code. Therefore, we can check its source code to verify the vulnerabilities. Second, since a large number of firmware images do not have source code,  static analysis is an acceptable method to verify the vulnerabilities in this case. Third, static analysis may fail to check several vulnerabilities that do not disclose the corresponding insecure codes. In this case, dynamic analysis can be used to make up for the shortcomings of static analysis. We here employ the firmware emulation technique \textit{FIRMADYNE} that proposed by Chen et al.~\cite{chen2016towards} to conduct dynamic analysis on firmware. 
% % \yuan{\color{red}How do you combine the dynamic and static analysis?}
% \noindent\textit{FIRMADYNE} dedicates to emulating the Linux-based firmware on desktop. It overcomes the general challenges in emulating firmware, such as the presence of hardware-specific peripherals, usage of nonvolatile memory, and creation of dynamically generated files. 
% Our evaluation method can confirm the true positive rate of our result, but hard to tell the false negative rate since several vulnerabilities may cannot be verified even with the source code audit.

% We first select XX firmware images which have a total of XX vulnerabilities that identified by \system, as shown in Table~\ref{Table: Accuracy Evaluation}. In consideration of our large-scale dataset, it is unrealistic to conduct analysis on each firmware image. Thus, we randomly select these firmware images based
% X of XX firmware images are from OpenWrt which have corresponding source codes. For these firmware images, we can review their source codes to verify the vulnerabilities.
% The other XX firmware images are without source codes. , static analysis  in these firmware images. 
% \yuan{\color{red}This section doesn't reads like an end-to-end evaluation. It is more like an experiment set up.}
% Though \system detects $128,757$ security vulnerabilities from $34,430$ firmwares, we still lack the ground truth that whether our results are correct. 
% We need to confirm our results in two aspects. First of all, we should confirm the TPCs we identified are really used in firmwares. 
% Second, we need to verify the corresponding vulnerabilities also exist. 
% For several vulnerabilities, we
% In fact, if we verify the vulnerabilities exist, we can 
% turn back confirm the corresponding TPCs exist as well.
% Thus, we can directly verify the identified vulnerabilities to evaluate the accuracy of \system.
% Since
% It is straightforward to review the source codes of firmware to verify the corresponding vulnerabilities. 
% Nevertheless, except for the firmware from OpenWrt, we cannot obtain the source codes for most vulnerable firmware. 
% In the absence of source codes, static analysis is an acceptable way to confirm our results. 
% However, it may still fail to check several vulnerabilities that do not disclose the corresponding insecure codes. Thus, we combine the dynamic analysis and static analysis to perform the evaluation. 


% For the vulnerabilities which have been po, we choose the static analysis to verify them. 
% At the same time, we will also rely on static analysis to determine whether the corresponding TPCs exist.
% For the vulnerabilities which have public Proof-of-Checks (PoCs), we will first emulate the corresponding firmware images and then use PoCs to test them. 
% For the vulnerabilities which have public PoCs, we adopt the dynamic analysis to verify them. For the remained vulnerabilities, we utilize static analysis to validate them.


% In consideration of our large-scale dataset, it is unrealistic to evaluate \system's accuracy on all firmware images. Therefore, we select some representative firmware according to two standards: 1) each identified vulnerability of the firmware has practical verification methods, whether through source code audit, static analysis, or dynamic analysis; and 2) include as many vendors and categories as possible.
% % We thus choose five firmwares, which are convenient to conduct static analysis and dynamic analysis, for this test.
% % \yuan{\color{red}How many images did you choose? Need to be specific. How do you choose them? If you are not doing a random sampling, people might say you are cherry picking results.} 
% We randomly select $35$ firmware images which have a total of $382$ vulnerabilities that identified by \system, as shown in Table~\ref{Table: Accuracy Evaluation}. $5$ out of the $35$ firmware images are from OpenWrt which have the corresponding source code. For these firmware images, we adopt source code audit to verify the vulnerabilities.
% The other $30$ firmware images are without source codes. We check the vulnerabilities in them either through static analysis or dynamic analysis.
% We have two standards to choose these five firmware images. First of all, we select the Linux based firmware since \textit{FIRMADYNE}  only supports emulating the firmware developed on Linux. Then, each identified vulnerability of the firmware has practical verification methods, either through static analysis or dynamic analysis.

% \textbf{TPCs Verification.}   For the TPCs verification, we need to both confirm that we find the real TPCs and the corresponding versions are also correct. Therefore, we first adopt static analysis by utilizing \textit{IDA Pro} to disassemble the firmwares to check each TPC manually. \textit{IDA Pro} is eligible to identify the common functions from  assembly codes, e.g., the functions in \textit{OpenSSL}, which can help us to identify the TPCs. Next, the verified vulnerabilities can turn back to assist us in identifying the TPCs. For example, several vulnerabilities only exist in specific versions of TPCs. Thus, if we confirm these vulnerabilities exist, we can also verify that the corresponding TPCs also exist well. We will discuss our vulnerabilities verification process in next paragraph. \yuan{I still feel the TPC validation process is not so convincing. Sometimes you use the code in the firmware, which would be good. However, sometimes you use the vulnerability, which might not be 100\% confident such vulnerability is caused by the TPC. Maybe it's better to drop validating TPC, and just write that you use both static analysis and dynamic analysis to confirm the vulnerability.}

% As shown in Table~\ref{Table: Accuracy Evaluation}, we have verified the TPCs involved in each firmware. For TPCs detected by \system, we confirm that they all really exist in corresponding firmwares and the versions of TPCs are also correct. In other words, we achieve $100\%$ accuracy in identifying TPCs with correct versions.




% \noindent\textbf{Vulnerabilities Verification.}   
% \textbf{First}, we  audit the source code of the firmware from OpenWrt. According to the result, \system reaches $100\%$ accuracy in identifying the $47$ vulnerabilities from these firmware images. \textbf{Second}, we combine static analysis and dynamic analysis to evaluate the remaining firmware images. We first manually review the disclosure reports of the $335$ vulnerabilities in the $30$ firmware images to determine the appropriate verification methods for each vulnerability. Then, we divide the $335$ vulnerabilities into two parts according to their corresponding verification method.
% $192$ vulnerabilities in the first part can be verified through static analysis and $143$ vulnerabilities in the second part can be validated by dynamic analysis. 
% % We carefully review the description of each vulnerability on CVE website~\cite{CVE} to determine which method is most 
% % For the vulnerabilities which have been pointed out the vulnerable function codes, we choose the static analysis to verify them. 
% % % At the same time, we will also rely on static analysis to determine whether the corresponding TPCs exist.
% % For the vulnerabilities which have public Proof-of-Checks (PoCs), we will first emulate the corresponding firmwares and then use PoCs to test them. 
% % % The vulnerabilities which are confirmed by PoC checking method also can turn back to confirm the corresponding TPCs exist as well. 
% \textbf{Third}, we adopt \textit{IDA} to conduct static analysis to verify the vulnerabilities in the first part.
% % we verify all the vulnerabilities based on static analysis and dynamic analysis. We first adopt the \textit{IDA Pro} to conduct static analysis on firmware to verify the vulnerabilities in the first part.
% Based on our previous report review, we confirm the vulnerable code snippets for involved vulnerabilities. We then disassemble the firmware and manually check the vulnerable code snippets from assembly codes. 
% % \yuan{\color{red}This seems to be quite similar to the third-party library identification, so I propose to merge them and only talk about vulnerability validation.}
% % In addition, \textit{IDA Pro} is eligible to identify the common functions from  assembly codes, which greatly reduces our manual work. We 
% \textbf{Finally}, we use  \textit{FIRMADYNE} to emulate the firmware which has vulnerabilities that should be verified through dynamic analysis. 
% Since different firmware varies greatly, it requires a lot of manual work to configure each firmware image to meet the emulating requirements. After successfully emulating the involved firmware, we reproduce PoCs for the second part's vulnerabilities and utilize them to attack the running emulated firmware. For the PoC which takes effect, we regard its corresponding vulnerability exists.

% % Though all the tested firmware are based on the Linux system, we cannot simply emulate them without any additional configuration.  Manual modification is needed on a case by case basis. Therefore, we pay a lot of manual work on emulating these firmware images and modify the configuration for each firmware image. We then utilize the PoCs to verify the vulnerabilities of emulated firmware in the second part.

% In summary, we manually verify a total of $382$ vulnerabilities and confirm $368$ vulnerabilities really exist.
% % \system reaches $xx$ accuracy in identifying vulnerabilities . 
% We fail to verify $14$ vulnerabilities in four firmware images, with one from TP-Link, and the other three from TSmart. Overall, \system achieves an average of $96.3\%$ accuracy in identifying the vulnerabilities caused by TPCs in firmware.


% \system reaches $100\%$ accuracy in identifying the vulnerabilities in the other four firmware except for the firmware from TSmart. \system detects $20$ vulnerabilities in TSmart's firmware where $3$ vulnerabilities are caused by BusyBox and $17$ vulnerabilities are caused by OpenSSL. However, we fail to verify $3$ high-risk vulnerabilities caused by OpenSSL. We further conduct an in-depth analysis of TSmart's firmware. We find TSmart has manually fixed up these three vulnerabilities rather than updates to the newest version. The results reflect that TSmart already has the awareness to check the vulnerabilities of TPCs. They choose to manually repair the high-risk vulnerabilities rather than simply update the TPC to the latest version due to that the newest TPC may cause other potential problems which will also bring inconvenient for development.



% We further Except for the firmware from \textit{Tuya},   What's more, all the TPCs that \system detected are actually used in firmwares. We further 


% we can review their 
% We implement the Proof-of-Check (PoC) for XX security vulnerabilities that caused by xx CVEs. For the 


% We conduct the evaluation in three steps.
% First of all, we review the description of each vulnerability to confirm the


% We utilize the \textit{IDA Pro} to analyze these firmwares. First of all, we extract





% Thus, we select static analysis is an alternative method to check the vulnerabilities.

% We implement our experiment in three steps. First of all, we select $xx$ firmwares which have been reported vulnerable by \system. Since static analysis involves a lot of manual work, we only choose a few representative firmwares from each vendor.

% Next, we review the description of each vulnerability. 


% Next, we use the \textit{IDA Pro} to disassemble each firmware. We do not directly disassemble the whole firmware. We first extract the files from firmware. Then, we locate the vulnerable library files and disae


% However, it is challenging to get the ground truth for two reasons.  First of all, we cannot obtain the source codes for most vulnerable firmwares, except for several firmwares from OpenWrt. Without source codes, it is hard to check the vulnerabilities just by static analysis of disassembly codes. Second, it is difficult to get feedback if we check the vulnerabilities on real IoT devices since most vulnerabilities may not affect the running of IoT devices. It is also hard to check whether the real IoT devices are using the exact firmwares that we want to test.
% % since we cannot obtain the source codes of vulnerable firmwares or check on real vulnerable IoT devices.

% % The most straightforward method is to check the source codes of vulnerable firmwares.
% % Nevertheless, it is hard to check them since we cannot get the source codes except for the firmwares from OpenWrt. What's more, we lack the corresponding vulnerable IoT devices due to our limited budget.
% % What's more, without real devices, we cannot implement the vulnerabilities to test the corresponding devices we identified 
% % which will raise serious ethical issues.
% Regarding these two challenges, we mainly utilize the \textit{FIRMADYNE} to emulate the firmwares on desktop and then manually test each vulnerability.  \textit{FIRMADYNE} was proposed by Chen et al.~\cite{chen2016towards} that dedicates to emulating the Linux based firmwares on desktop. It overcomes the general challenges in emulating firmwares, such as the presence of hardware-specific peripherals, usage of nonvolatile memory, and creation of dynamically generated files. 
% By emulating the firmwares on the local desktop, we can avoid to purchase the real IoT devices and can confirm that we are analyzing the correct firmwares.
% % easily observe whether the vulnerabilities really exist with the help of some professional tools, e.g., Wireshark~\cite{Wireshark}.

% We conduct our experiment in three steps.
% First of all, we select a total of $5$ representative firmwares which are developed based on Linux, as shown in Table~XXX. Since we need to manually check the vulnerabilities for each vulnerability, we select the firmwares which contain relatively few vulnerabilities.

% Next, we use the \textit{FIRMADYNE} to emulate these firmwares. Though all the tested firmwares are based on Linux system, we cannot simply emulate them without any additional configuration.  Manual modification is needed on a case by case basis. Therefore, we pay a lot of manual work on emulating these firmwares and modify the configuration for each firmware. 

% Finally, we conduct a detailed investigation of the vulnerabilities involved and implement proof-of-concept (PoC) for a total of $124$ security vulnerabilities respectively. Our results indicate that $94\%$ of the detected security vulnerabilities really exists. 





% \begin{table*}[]
% \centering
% % \large
% \tiny

% \renewcommand\arraystretch{1.0}
% \caption{Comparison of \textit{\system}, \cite{costin2014large}, \textit{360} and \textit{Alibaba}.}
% \label{Table: Comparison}
% \vspace{-5mm}
% \resizebox{\textwidth}{
% % \Rotatebox{90}{%

% \begin{tabular}{cccccclccclccclccc}
% \hline \hline
% \multirow{2}{*}{Vendor} &
%   \multirow{2}{*}{Category} &
%   \multirow{2}{*}{Firmware} &
%   \multicolumn{3}{c}{\system} &
%   &
%   \multicolumn{3}{c}{
% binaré\cite{costin2014large, binare}} &
%   &
%   \multicolumn{3}{c}{\textit{360}~\cite{360iot}} &
%   &
%   \multicolumn{3}{c}{\textit{Alibaba}~\cite{aliiot}} \\ \cline{4-6} \cline{8-10} \cline{12-14} \cline{16-18} 
%  &
%   &
%   &
%   \# TPC &
%   \# Vul. &
%   Time (s) &
%   &
%   \# TPC &
%   \# Vul. &
%   Time (s) &
%   &
%   \# TPC &
%   \# Vul. &
%   Time (s) &
%   &
%   \# TPC &
%   \# Vul. &
%   Time (s) \\ \hline
% D-Link   & Router     & 3001\_DIR885LA1.bin    & \textbf{17} & \textbf{124} & \textbf{4} &  & 12 & 69 & 420 &  & 4  & 7            & 60 &  & 7  & 90           & 47    \\
% D-Link   & Camera     & dcs-935l\.bin          & \textbf{9}  & 57           & \textbf{3} &  & 5  & 56  & 300 &  & 1  & 1            & 60 &  & 5  & \textbf{78}  & 44    \\
% D-Link   & Router     & dir895la1.bin          & \textbf{17} & 114         & \textbf{3} &  & 11 & 113 & 300 &  & 6  & \textbf{173} & 60 &  & 7  & 96           & 20    \\
% TP-Link  & Router     & c7v5.bin               & \textbf{19} & \textbf{146} & \textbf{4} &  & 12 & 119 & 420 &  & 7  & 10           & 60 &  & NA & NA           & 47    \\
% TP-Link  & Router     & c2600v1.bin            & \textbf{31} & \textbf{148} & \textbf{9} &  & 12 & 119 & 480 &  & 10 & 99           & 60 &  & 1  & 1            & 209   \\
% TP-Link  & Router     & archer\_a7(eu).bin      & \textbf{18} & \textbf{123} & \textbf{4} &  & 11 & 96 & 240 &  & 7  & 88           & 60 &  & NA & NA           & 53    \\
% TP-Link  & Router     & ad7200v2.bin           & \textbf{30} & \textbf{140} & \textbf{5} &  & 12 & 114 & 360 &  & 10 & 99           & 60 &  & 1  & 1            & 220   \\
% TP-Link  & Router     & e4r.bin                & \textbf{15} & 106           & \textbf{3} &  & 11 & 89 & 300 &  & 5  & \textbf{228} & 60 &  & 1  & 0            & 31    \\
% TP-Link  & Router     & p7 1.0\_en\_1.2.0.bin  & \textbf{14}  & \textbf{101}  & \textbf{3} &  & 8  & 72  & 300 &  & 4  & 69           & 60 &  & NA & NA           & 68    \\
% TP-Link  & Camera     & tl-ipc423(p).bin       & \textbf{15}  & 124           & \textbf{2} &  & 4  & 114 & 300 &  & 5  & 9            & 60 &  & 6  & \textbf{135} & 176   \\
% TP-Link  & Camera     & tl-ipc543k(p).bin      & \textbf{14}  & 106           & \textbf{2} &  & 4  & 105 & 240 &  & 4  & 7            & 60 &  & 6  & \textbf{135} & 60    \\
% Trendnet & Router     & luci-ar71xx.bin        & \textbf{14} & \textbf{104} & \textbf{4} &  & 8  & 85  & 300 &  & NA & NA           & 60 &  & NA & NA           & 46    \\
% Trendnet & Router     & tew755ap.bin           & \textbf{24} & 141          & \textbf{5} &  & 8  & 114 & 360 &  & 4  & 78           & 60 &  & 13 & \textbf{330} & 32    \\
% Trendnet & Switch     & tl2-g244-all.hex       & \textbf{4}  & \textbf{48}  & \textbf{3} &  & 4  & 27  & 240 &  & 1  & 6            & 60 &  & 1  & 42           & 51    \\
% Dahua    & Camera     & wifimac\_upall.bin     & \textbf{15} & \textbf{111}  & \textbf{3} &  & 8  & 84  & 240 &  & 7  & 40           & 60 &  & 1  & 1            & 28    \\
% Xiaomi   & Router     & miwifi\_r1cm\_all.bin  & \textbf{16} & 128          & \textbf{7} &  & 7  & 100  & 360 &  & 7  & \textbf{176} & 60 &  & NA & NA           & 66    \\
% Xiaomi   & Router     & miwifi\_all\_bd6da.bin & \textbf{16} & \textbf{116} & \textbf{5} &  & 8  & 88  & 360 &  & 7  & 84           & 60 &  & NA & NA           & 32    \\
% TSmart   & Camera & ymsmart-2.0.2.bin      & \textbf{7}  & \textbf{131} & \textbf{5} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & 6  & 131          & 1,977 \\
% TSmart   & Camera & lcipc-consumer.bin     & \textbf{5}  & \textbf{102}  & \textbf{3} &  & 2  & 11  & 300 &  & 2  & 9            & 60 &  & 2  & 14           & 78    \\
% TSmart   & Light      & XR871_SAMPLE_QIO_1.1.1.BIN  & \textbf{1}          & \textbf{27}           & \textbf{2} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 34    \\ \hline 
% % & & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ & \# $\overline{Time(s)}$ &
%  & Average Results & & \textbf{15.8} & \textbf{114.2} & \textbf{4.2} & & 7.7 & 82.9 & 303 & & 4.8 & 62.3 & 60 & & 3 & 55.5 & 174.7 & \hline \hline
% \end{tabular}
% % }%
% }
% \end{table*}



\begin{table*}[]
\centering
% \large
\tiny

\renewcommand\arraystretch{1.0}
\setlength\tabcolsep{4.5pt}
\caption{Comparison of \textit{\system}, \textit{binaré}, \textit{360 FirmwareTotal}, and \textit{Alibaba FSS}.}
\label{Table: Comparison}
% \vspace{-5mm}
\resizebox{\textwidth}{
% \Rotatebox{90}{%

\begin{tabular}{ccccccclccclccclccc}
\hline \hline
\multirow{2}{*}{Vendor} &
  \multirow{2}{*}{Category} &
  \multirow{2}{*}{Firmware} &
  \multirow{2}{*}{OS Support} &
  \multicolumn{3}{c}{\system} &
   &
  \multicolumn{3}{c}{
\textit{binaré}\cite{binare}} &
   &
  \multicolumn{3}{c}{\textit{360 FirmwareTotal}~\cite{360iot}} &
   &
  \multicolumn{3}{c}{\textit{Alibaba FSS}~\cite{aliiot}} \\ \cline{5-7} \cline{9-11} \cline{13-15} \cline{17-19} 
 &
   &
   &
   &
  \# TPC &
  \# Vul. &
  Time (s) &
   &
  \# TPC &
  \# Vul. &
  Time (s) &
   &
  \# TPC &
  \# Vul. &
  Time (s) &
   &
  \# TPC &
  \# Vul. &
  Time (s) \\ \hline
D-Link   & Router     & 3001\_DIR885LA1.bin & \textcolor{green}{\checkmark}   & \textbf{17} & \textbf{124} & \textbf{9} &  & 12 & 69 & 420 &  & 4  & 7            & 60 &  & 7  & 90           & 47    \\
D-Link   & Camera     & dcs-935l\.bin  & \textcolor{green}{\checkmark}        & \textbf{11}  & 65           & \textbf{7} &  & 5  & 56  & 300 &  & 1  & 1            & 60 &  & 5  & \textbf{78}  & 44    \\
D-Link   & Router     & dir895la1.bin  & \textcolor{green}{\checkmark}        & \textbf{17} & 114         & \textbf{9} &  & 11 & 113 & 300 &  & 6  & \textbf{173} & 60 &  & 7  & 96           & 20    \\
TP-Link  & Router     & c7v5.bin    & \textcolor{green}{\checkmark}           & \textbf{19} & \textbf{146} & \textbf{6} &  & 12 & 119 & 420 &  & 7  & 10           & 60 &  & NA & NA           & 47    \\
TP-Link  & Router     & c2600v1.bin   & \textcolor{green}{\checkmark}         & \textbf{31} & \textbf{148} & \textbf{9} &  & 12 & 119 & 480 &  & 10 & 99           & 60 &  & 1  & 1            & 209   \\
TP-Link  & Router     & archer\_a7(eu).bin  & \textcolor{green}{\checkmark}    & \textbf{18} & \textbf{123} & \textbf{6} &  & 11 & 96 & 240 &  & 7  & 88           & 60 &  & NA & NA           & 53    \\
TP-Link  & Router     & ad7200v2.bin  & \textcolor{green}{\checkmark}         & \textbf{30} & \textbf{140} & \textbf{8} &  & 12 & 114 & 360 &  & 10 & 99           & 60 &  & 1  & 1            & 220   \\
TP-Link  & Router     & e4r.bin  & \textcolor{green}{\checkmark}              & \textbf{15} & 106           & \textbf{8} &  & 11 & 89 & 300 &  & 5  & \textbf{228} & 60 &  & 1  & 0            & 31    \\
TP-Link  & Router     & p7 1.0\_en\_1.2.0.bin & \textcolor{green}{\checkmark} & \textbf{14}  & \textbf{101}  & \textbf{5} &  & 8  & 72  & 300 &  & 4  & 69           & 60 &  & NA & NA           & 68    \\
TP-Link  & Camera     & tl-ipc423(p).bin  & \textcolor{green}{\checkmark}     & \textbf{16}  & 125           & \textbf{5} &  & 4  & 114 & 300 &  & 5  & 9            & 60 &  & 6  & \textbf{135} & 176   \\
TP-Link  & Camera     & tl-ipc543k(p).bin  & \textcolor{green}{\checkmark}    & \textbf{14}  & 106           & \textbf{7} &  & 4  & 105 & 240 &  & 4  & 7            & 60 &  & 6  & \textbf{135} & 60    \\
Trendnet & Router     & luci-ar71xx.bin   & \textcolor{green}{\checkmark}     & \textbf{15} & \textbf{107} & \textbf{9} &  & 8  & 85  & 300 &  & NA & NA           & 60 &  & NA & NA           & 46    \\
Trendnet & Router     & tew755ap.bin    & \textcolor{green}{\checkmark}       & \textbf{24} & 141          & \textbf{5} &  & 8  & 114 & 360 &  & 4  & 78           & 60 &  & 13 & \textbf{330} & 32    \\
Trendnet & Switch     & tl2-g244-all.hex  & \textcolor{green}{\checkmark}     & \textbf{4}  & \textbf{48}  & \textbf{8} &  & 4  & 27  & 240 &  & 1  & 6            & 60 &  & 1  & 42           & 51    \\
Dahua    & Camera     & wifimac\_upall.bin  & \textcolor{green}{\checkmark}   & \textbf{15} & \textbf{111}  & \textbf{6} &  & 8  & 84  & 240 &  & 7  & 40           & 60 &  & 1  & 1            & 28    \\
Xiaomi   & Router     & miwifi\_r1cm\_all.bin & \textcolor{green}{\checkmark} & \textbf{16} & 128          & \textbf{7} &  & 7  & 100  & 360 &  & 7  & \textbf{176} & 60 &  & NA & NA           & 66    \\
Xiaomi   & Router     & miwifi\_all\_bd6da.bin & \textcolor{green}{\checkmark} & \textbf{16} & \textbf{116} & \textbf{5} &  & 8  & 88  & 360 &  & 7  & 84           & 60 &  & NA & NA           & 32    \\
TSmart   & Camera & ymsmart-2.0.2.bin  & \textcolor{green}{\checkmark}    & \textbf{8}  & \textbf{133} & \textbf{5} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & 6  & 131          & 1,977 \\
TSmart   & Camera & lcipc-consumer.bin  & \textcolor{green}{\checkmark}   & \textbf{5}  & \textbf{102}  & \textbf{3} &  & 2  & 11  & 300 &  & 2  & 9            & 60 &  & 2  & 14           & 78    \\
TSmart   & Light      & XR871\_QIO\_1.1.1.bin & \textcolor{red}{\XSolidBrush} & \textbf{1}          & \textbf{27}           & \textbf{8} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 34    \\

TSmart   & Light      & esp\_warm\_light\_1.1.0.bin & \textcolor{red}{\XSolidBrush} & \textbf{1}          & \textbf{2}           & \textbf{7} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 55    \\ 
TSmart   & Doorbell    & DOORBELL-2.0.3.20180425.bin & \textcolor{red}{\XSolidBrush} & \textbf{1}          & \textbf{16}           & \textbf{8} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 49    \\  
TSmart   & Plug      & esp\_12F\_xw\_plug\_1.0.5.bin & \textcolor{red}{\XSolidBrush} & \textbf{1}          & \textbf{36}           & \textbf{9} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 21    \\ 
TSmart   & Plug      & SIG-WITHOUTSYS\_0.0.16.bin & \textcolor{red}{\XSolidBrush} & \textbf{1}          & \textbf{36}           & \textbf{7} &  & NA & NA  & 120 &  & NA & NA           & 60 &  & NA & NA           & 42    \\
 \hline 
% & & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ &  $\overline{Time(s)}$ & & \# $\overline{3rd \ P.C.}$ & \# $\overline{Vul.}$ & \# $\overline{Time(s)}$ &
%  & Average Results of 19 Linux-based Firmware Images & &  & \textbf{15.8} & \textbf{114.2} & \textbf{4.2} & & 7.7 & 82.9 & 303 & & 4.8 & 62.3 & 60 & & 3 & 55.5 & 174.7 & \hline 
\hline
\end{tabular}
% }%
}
\vspace{-1em}
\end{table*}


\vspace{-0.3cm}
\subsection{Comparison With Academic and Industry State of the Arts}
\label{section: performance measurement}
% The \system achieves great results in matching the TPCs and identifying the N-days vulnerabilities from $34,430$ firmwares.
% Though multiple static analysis methods are proposed to detect the vulnerabilities in the firmware, we cannot compare \system with all of them. Most of these methods require two inputs: . In this paper, we compare which are still working now.
% Besides, there are several companies also provide commercial tools that claim to detect the N-days vulnerabilities caused by TPCs from the firmware and most of these tools are still in test.

\noindent\textbf{Comparative Analysis With Academic Works.}  We compare \system with three academic works: \textit{Gemini}~\cite{xu2017neural}, \textit{BAT}~\cite{hemel2011finding} and \textit{OSSPolice}~\cite{duan2017identifying}. The original \textit{Gemini} uses 8 block-level attributes to conduct code similarity comparison. We enhance it with our CFG weight-based method to detect the TPCs in firmware. 
\textit{BAT} leverages string literals to identify the TPCs in binaries, but cannot detect the exact versions. \textit{OSSPolice} is originally designed to detect the open-source software usage at version-level in Android apps. Given it supports finding TPCs in C/C++ native libraries, we successfully apply it on IoT firmware and compare it with \system. Before we conduct comparison, we generate the corresponding TPC database for \textit{BAT} and \textit{OSSPolice} based on their instructions respectively.
Table~\ref{Table: Academic Comparison} presents the comparison results of \system with \textit{Gemini}, \textit{BAT}, and \textit{OSSPolice}. We do not report the results of \textit{BAT} at version-level since it does not support version-level identification. For TPC-level identification, \system is far better than other tools. \system reports more TPCs at a higher precision and recall rate. For version-level identification, \system outperforms \textit{Gemini} and \textit{OSSPolice} on both metrics. We further explore the reasons that why \system is better than other tools. First, \textit{Gemini} ignores the function-level attributes which offer much useful information on the structure of CFGs. Second, \textit{BAT} mainly utilizes string literals to identify the TPCs. It uses the direct feature matching to compare the string literals extracted from TPCs and firmware, which causes a low precision and recall rate. Finally, \textit{OSSPolice} utilizes a hierarchical matching strategy, which relies on the package structures of TPCs, to identify TPCs. Nevertheless, the package structures of the same TPC in different versions can be easily changed. 
Besides, its feature extraction tool does not perform well on IoT firmware since it is not optimized for firmware.



\noindent\textbf{Comparative Analysis With Industry Systems.} We compare \system with
% one academic incubated system:  \textit{binaré}~\cite{costin2014large, binare} and
three commercial systems: \textit{binaré}~\cite{binare}, \textit{360 FirmwareTotal}~\cite{360iot}, and \textit{Alibaba FSS}~\cite{aliiot}. \textit{binaré} is actually developed from a state-of-the-art work~\cite{costin2014large}. The prototype system proposed in \cite{costin2014large} did not support finding the TPCs and the corresponding vulnerabilities in firmware while its commercial version supports this function. \textit{360} and \textit{Alibaba} are two well-known companies worldwide, and both have much experience in IoT security. They are the few that offer publicly accessible systems that can detect the vulnerability caused by TPCs in firmware.  \textit{binaré} and \textit{FirmwareTotal} offer free trials and \textit{FSS} costs \$300 for each usage. 

Since these commercial systems may directly analyze the configuration files in OpenWrt firmware to identify the TPCs, we compare them on commercial firmware images.
We mainly compare their performance in identifying the TPCs and corresponding vulnerabilities in firmware. As shown in Table~\ref{Table: Comparison}, we select 24 firmware images include 19 Linux-based firmware images and $5$ monolithic firmware images to test the four systems. The analysis results are as follows.
% We do not compare \system with other academic works due to the following reasons. (1) Though there are some systems~\cite{backes2016reliable,duan2017identifying,zhang2019libid} that have been proposed to detect the TPCs used in Android apps, they cannot analyze the IoT firmware. These systems require Android features support. (2) Since developing a new fine-grained analysis tool is not the main focus of this work, we adopt a state-of-the-art \textit{Gemini} and do not compare it with similar 
% tools~\cite{feng2016scalable,david2018firmup,ding2019asm2vec}.
% are fine-grained. The previous work of static analysis and dynamic analysis was mainly to detect some specific vulnerabilities, which is different from the purpose of our coarse-grained analysis method based on version checking. Since the fine-grained method integrated in \system is based on an existing, we do not compare it with
% There are some systems that have been proposed to detect the TPCs used in Android apps. Nevertheless, they cannot analyze the IoT firmware since they use multiple features of Android. Constin et al.~\cite{costin2014large} has proposed a prototype system to analyze the first large-scale analysis of the security of IoT firmware. However
% The static and dynamic methods proposed by previous works 
% There are some systems have been proposed to detect the TPCs used in Android apps.
% Constin et al.~\cite{costin2014large} has conducted the first large-scale analysis of the security of IoT firmware. Though they , their prototype system actually cannot find the TPCs and the corresponding vulnerabilities in firmware. We finally
% However, since they are designed . We finally compare three commercial systems:. \textit{binaré} is actually developed from a state-of-art work~\cite{costin2014large}. The prototype system proposed in \cite{costin2014large} cannot find the TPCs and the corresponding vulnerabilities in firmware. Therefore, we utilize its commericial version \textit{binaré} instead. \textit{360} and \textit{Alibaba} are two well-known companies worldwide, and both have much experience in IoT security. They are the few that offer publicly accessible systems that can detect the vulnerability caused by TPCs in firmware.  \textit{360} offers unlimited free trials while \textit{Alibaba} offers only one free trial. We purchase $24$ extra usage times of \textit{Alibaba} which costs $\$6,000$.
% In this subsection, we compare our system with a state-of-the-art work~\cite{costin2014large} and two commercial systems from \textit{360}~\cite{360iot} and \textit{Alibaba}~\cite{aliiot} in four aspects: the number of successfully analyzed firmware images, the number of detected TPCs, the number of identified vulnerabilities, and the analysis time. 
% To the best of our knowledge, there is no previous work . Though \cite{costin2014large}
% Though multiple works have proposed methods to detect the vulnerabilities in firmware, most of them lack prototype systems and source code. Besides, some methods based on code similarity comparison are not suitable to compare with \system since they require providing assembly code of each vulnerability.  
% Thus, we finally choose to compare with \cite{costin2014large} which provides a prototype system that has similar functions to \system. On the other hand, \textit{360} and \textit{Alibaba} are two well-known companies worldwide, and both have much experience in IoT security. They are the few that offer publicly accessible systems that can detect the vulnerability caused by TPCs in firmware.  \textit{360} offers unlimited free trials while \textit{Alibaba} offers only one free trial. We purchase $20$ extra usage times of \textit{Alibaba} which costs $\$6,000$.
% As shown in Table~\ref{Table: Comparison}, we select $20$ firmware images randomly from six vendors as test cases. Since \system, \textit{360} and \textit{Alibaba} all skip the vulnerabilities of the Linux kernel, we also exclude this part of result from \cite{costin2014large} for fairness.
% According to our results, \system outperforms the other three systems in all aspects. 
\textbf{First}, \system can analyze all test firmware images and is the only one that supports analyzing monolithic firmware. For the 19 Linux-based firmware images,  \textit{binaré} is unable to process $1$ firmware images, \textit{FirmwareTotal} cannot deal with $2$ firmware images, and \textit{FSS} fails to analyze $7$ firmware images.
% Those Linux-based firmware images that cannot be analyzed by \textit{360} and \textit{Alibaba} do not adopt the traditional filesystems which increase the difficulty of analysis.
% In addition, to measure the performance of \system comprehensively, we specially select a firmware image from TSmart which cannot be analyzed by \system, as shown in the last line of Table~\ref{Table: Comparison}. \cite{costin2014large}, \textit{360}, and \textit{Alibaba} also fail to analyze this firmware. 
% To explore the reasons behind, we use the \textit{IDA Pro} to conduct static analysis on this firmware. Based on our result, we find this firmware is just composed of pieces of function codes. We do not detect any TPCs from this smart home device.
\textbf{Second}, 
% compared with the other three systems, 
\system detects the most TPCs in each test case. The TPCs discovered by \system have covered all the results of \textit{binaré}, \textit{FirmwareTotal} and \textit{FSS}.
% We conclude the excellent performance of \system to three reasons: 1) \system conducts a more thorough extraction of firmware. Since \system contains a custom extraction tool, it extracts more objects from firmware that keep more information.  2) \system maintains a large-scale TPC list. 
We notice that the results from \textit{binaré}, \textit{FirmwareTotal} and \textit{FSS} mainly contain several popular TPCs, e.g., BusyBox and OpenSSL,  while \system can detect some uncommon TPCs, e.g., libogg. 
% 3) \system adopts an effective matching algorithm. 
% \system maintains a large-scale TPC list and adopts a custom matching algorithm, . The system 
% \textit{Alibaba} does not achieve a great performance in detecting the TPCs since it 
% % The \system maintains a large scale vulnerability list to match the TPCs in firmwares.
% % \system has discovered all the TPCs with the same version that reported by \textit{360} and \textit{Alibaba}. Since \system maintains a large-scale TPC list and adopts a custom matching algorithm, it discovers 
% %  it discovers more TPCs which contain confirmed N-days vulnerabilities than 360 and \textit{Alibaba}.
\textbf{Third}, \system identifies more N-days vulnerabilities in $12$ of the $19$ Linux-based firmware images in comparison with the other three systems. We conclude two reasons that why \system detects fewer vulnerabilities than other systems in the other 7 test cases. (1) \textit{binaré}, \textit{FirmwareTotal}, and  \textit{FSS} incorrectly report N-days vulnerabilities not belonging to the corresponding firmware. (2) For several cases, they report multiple versions of the same TPCs. For example, \textit{FSS} reports two different versions of OpenSSL in tl-ipc423(p).bin, and calculates the vulnerabilities according to these two versions. We further remove the above false positives of other systems in these 7 test cases and find \system can detect more N-days vulnerabilities than them in all cases.
% \system mainly depends on our vulnerability database that builds on CVE Detail~\cite{cvedetail}. 
% In  the remaining $7$ test cases, \textit{360} detects more vulnerabilities in $3$ test cases while \textit{Alibaba} discovers more vulnerabilities in $4$ test cases.
% Though \system detects more TPCs, which contain all the TPCs with the same versions that discovered by \textit{360} and \textit{Alibaba}, in these $7$ test cases, \system still find fewer vulnerabilities than them. 
% % \yuan{\color{red}Again, be specfic about the results.}
% We conduct in-depth analysis and find two reasons for the results for these 7 test cases. First, \textit{Alibaba} and  \textit{360} incorrectly report N-days vulnerabilities not belonging to the corresponding firmware. 
% % by carefully checking the vulnerabilities that they discovered in these $7$ test cases.  
% Second, we discover that \textit{360} and \textit{Alibaba} maintain more detailed vulnerability databases than ours. For example, for the firmware of  tew755ap.bin from Trendnet, \system and \textit{Alibaba} both detect the \textit{tcpdump} used in  it. Nevertheless, our vulnerability database only has the corresponding CVEs from 2018 to 2019 while \textit{Alibaba} reports the vulnerability since 2014. 
% Therefore, we conduct further study to ensure the fairness of our experiments. We use our vulnerability database for  other three systems. The vulnerabilities found by \textit{360} and \textit{Alibaba} decreased dramatically after we change the vulnerability database, and \cite{costin2014large} does not change a lot. With the same vulnerability database, \system discovers more  since we can detect more TPCs. Besides, though our database is not as detailed as theirs, we can dynamically update the database by tracking the latest disclosed vulnerabilities.
\textbf{Finally}, \system spends less time when analyzing firmware. We implement \system on an Ubuntu server equipped with the i7-9700K CPU, RTX 2080 GPU, and 32 GB memory. 
\system analyzes each firmware image in less than 10 seconds which is much quicker than other systems in all test cases. 

% For each firmware image, \textit{360} spends 60 seconds to analyze it. \textit{binaré} spends an average of  303 seconds processing each firmware image.
% \textit{Alibaba} has an unstable performance on analyzing firmware where the best case is 20 seconds and the worst case is 33 minutes.

Overall, our results show that \system has a much better performance
than state-of-the-art tools from academia and commercial tools from industry. \system has a higher precision and recall than \textit{Gemini}, \textit{BAT}, and \textit{OSSPolice} at TPC-level and version-level.
In comparison with \textit{binaré}, \textit{FirmwareTotal}, and \textit{FSS}, \system achieves a higher success rate in analyzing firmware with less time, and can detect more TPCs, as well as identify more vulnerabilities.



% \begin{table*}[]
% \centering
% \caption{Accuracy Evaluation of \system}
% \renewcommand\arraystretch{0.9}
% \label{Table: Accuracy Evaluation}
% \begin{tabular}{ccccccc}
% \hline \hline
% Vendor &
%   Category &
%   firmware &
% %   \begin{tabular}[c]{@{}c@{}}\#  Third-party\\ Components\end{tabular} &
%   \# Vul. &
% %   \begin{tabular}[c]{@{}c@{}}\# Verified\\ TPCs\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}\# Verified\\ Vul.\end{tabular} \\ \hline
% Trendnet & Router & openwrt-ar71xx-generic-tew-823dru-squashfs-factory.bin             & 21  & 21 \\
% Trendnet & Router & tew-654tr\_a1\_fw100b19.bin                                        & 19  & 19 \\
% TP-Link  & Router & wr810nv2\_eu\_3\_16\_9\_up\_boot(160509).bin                       & 24  & 24 \\
% TSmart     & Camera & ipcam.20190314.v02.bin                                             & 20  & 14 \\
% Xiongmai & Camera & xmjp\_liteos\_hi3518ev200\_8188eu\_v1.01.liteos.20170630\_all.bin  & 24  & 24 \\ \hline \hline
% \end{tabular}
% \end{table*}










